On-manifold Adversarial Data Augmentation Improves Uncertainty Calibration

Uncertainty estimates help to identify ambiguous, novel, or anomalous inputs, but the reliable quantification of uncertainty has proven to be challenging for modern deep networks. In order to improve uncertainty estimation, we propose On-Manifold Adversarial Data Augmentation or OMADA, which specifically attempts to generate the most challenging examples by following an on-manifold adversarial attack path in the latent space of an autoencoder-based generative model that closely approximates decision boundaries between two or more classes. On a variety of datasets as well as on multiple diverse network architectures, OMADA consistently yields more accurate and better calibrated classifiers than baseline models, and outperforms competing approaches such as Mixup, as well as achieving similar performance to (at times better than) post-processing calibration methods such as temperature scaling. Variants of OMADA can employ different sampling schemes for ambiguous on-manifold examples based on the entropy of their estimated soft labels, which exhibit specific strengths for generalization, calibration of predicted uncertainty, or detection of out-of-distribution inputs.

==> newdata/new_table.tex <==
\begin{table}[t!]
	\captionsetup{singlelinecheck=false}
	\begin{tabular}{lrrrrrr}
		\toprule
		CIFAR-10 & \multicolumn{3}{c|}{DenseNet}   &  \multicolumn{3}{c}{WRN} \\
		&     ACE &     ACC &      \multicolumn{1}{c|}{AUC} &    ACE &     ACC &     AUC \\
		\midrule
		 Base &  0.0319 &  92.768 &  \multicolumn{1}{r|}{0.9076}  &  0.0341 &  91.596 &  0.9022 \\
		 OMADA &  0.0138 &  94.530 &   \multicolumn{1}{r|}{0.9252}&  0.0208 &  95.772 &  0.9243 \\
		OMADA-H &  \textbf{0.0058} & 93.652  &    \multicolumn{1}{r|}{0.8913} &  \textbf{0.0172} &  95.150 &  0.9210 \\
		OMADA-U &  0.0260 &  93.890 &  \multicolumn{1}{r|}{0.9678} &  0.0274 &  95.446 &  0.9750 \\
		 OMADA-SE &  0.0273 &  \textbf{94.988} &  \multicolumn{1}{r|}{0.9741} &   0.0207 &  \textbf{96.022} &  \textbf{0.9833} \\
		 OMADA-SE-H &  0.0281 &  94.258 &  \multicolumn{1}{r|}{0.9119} &  0.0222 &  95.882 &  0.9643 \\
		 OMADA-SE -U &  0.0302 &  94.618 &   \multicolumn{1}{r|}{\textbf{0.9786}} &  0.0231 &  95.248 &  0.9346 \\
		\bottomrule
	\end{tabular}
	\caption{Performance of OMADA ablation methods on calibration (ACE), network accuracy (ACC), and outlier detection (AUC). -H refers to the respective hard label variant, -U refers to the respective uniform label variant. DN refers to DenseNet.  Bold entries indicate the best-performing method. We report the mean over $5$ independent runs for each method (std devs. can be found in the appendix).}
	\label{table1_ablations}
	\vspace{-0.5cm}
\end{table}







==> newsections.tex <==
\section{Discussion}

\textbf{Importance of the Generative Model}
OMADA relies on a meaningful approximation of the data manifold, which allows finding ambiguous examples that lie close to the class decision boundaries.
Utilizing GANs is currently the best suited solution for complex high dimensional data, and OMADA demonstrates a beneficial use of the learned latent space apart from realistic data synthesis.
GANs and other generative models are notorious for their training instability, but this is also a very active research field, where better tools and algorithms become available quickly, and more and more pre-trained models are made available.
In our case OMADA delivered the best results with the most realistic generative model, the state-of-the-art BigBi-GAN~\cite{bigbigan_donahue}, and using our principled targeted sampling provided more robust improvements across all networks and architectures than simpler techniques working in image space.
Hence,  we expect that both uncertainty estimates and accuracy will improve with even better generative models and better approximations of the manifolds that will become available in the future, without requiring changes to the sampling principles of OMADA.
In terms of computational complexity, the main costs are only incurred when initially training the generative model.
OMADA and the core idea is of course not limited to GANs, but can utilize any autoencoder-based generative model which might be better suited for other data modalities (e.g. VAEs~\cite{kingma2013autoencoding}, VAE-GAN~\cite{rosca2017variational} and VQ-VAE2~\cite{vqvae2}).

\textbf{Benefits of manifold-based calibration}
OMADA can be directly applied to any data modality for which a generative model can be trained, including text, time series, spectrograms, or point clouds, e.g. for radar or LIDAR data. 
Other methods such as Mixup~\cite{OnMixupTrainThul} perform linear interpolation in the image space, which is not feasible if the dimensionality of the data changes, and might result in meaningless intermediate images (e.g. when interpolating between spectra). CEDA~\cite{ReLUMHein} generates uniform random-noise images for calibration, but this might not be a good approximation of out-of-data samples for non-image data.

\textbf{Principled Sampling of Ambiguous Data Points}
OMADA's principled sampling technique for data augmentation maximizes the chances of sampling truly ambiguous on-manifold samples that improve calibration, as apposed to naive sampling (which has only a tiny chance of sampling points near the boundary).
The targeted on-manifold adversarial attack of OMADA deliberately samples novel training points with multiple class-specific features, sharing the characteristics of all neighboring classes.
By training the image-space classifiers on such ambiguous samples a high uncertainty in those regions is learned, rather than an over-confident prediction for a single class.



\textbf{Model-agnostic Calibration}
One striking observation of our experiments (e.g. Fig.~\ref{fig3_ace}) is that the calibration quality of all competing methods varies strongly if tested on different network architectures, whereas OMADA consistently ranks among the top performers.
We chose the tested model architectures because of their varying capacities, layer types (e.g. VGG's MLPs, Residual blocks in ResNeXt), and their different peak accuracies.
Different downstream tasks (e.g. semantic segmentation or object detection), different data modalities (e.g. point clouds or word embeddings), and different hardware constraints for embedded solutions might require different types of network architectures.
Therefore it is highly desirable to have a method which is agnostic to the diversity of network architectures found in practice. 



